Generalization Guarantees for Multi-item Profit Maximization: Pricing, Auctions, and Randomized Mechanisms

We study multi-item profit maximization when there is an underlying distribution over buyers' values. In practice, a full description of the distribution is typically unavailable, so we study the setting where the mechanism designer only has samples from the distribution. If the designer uses the samples to optimize over a complex mechanism class -- such as the set of all multi-item, multi-buyer mechanisms -- a mechanism may have high average profit over the samples but low expected profit. This raises the central question of this paper: how many samples are sufficient to ensure that a mechanism's average profit is close to its expected profit? To answer this question, we uncover structure shared by many pricing, auction, and lottery mechanisms: for any set of buyers' values, profit is piecewise linear in the mechanism's parameters. Using this structure, we prove new bounds for mechanism classes not yet studied in the sample-based mechanism design literature and match or improve over the best-known guarantees for many classes.

==> app-learning-theory.tex <==
The following theorem relating Rademacher complexity and pseudo-dimension is well-known, though we work out the precise constants for completeness.

\pseudimerad*

\begin{proof} To prove this theorem, we will use the notion of a \emph{covering number.}
\begin{definition}[Covering number]
Let $A \subset \R^N$ be a set of vectors. We define $N_p(\beta,A)$ to be the cardinality of the smallest set $A' \subset \R^N$ such that for all $a \in A$, there exists $a' \in A'$ such that $\sqrt[p]{\frac{1}{N}\sum_{i = 1}^N (a_i - a_i')^p} \leq \beta$. We say that such an $A'$ $\beta$-covers $A$ in the $p$-norm and that $N_p(\beta,A)$ is the $L_p$-norm covering number.
\end{definition}
 We can relate the above definition to a mechanism class $\pazocal{M}$ over a set of samples $\sample = \left\{\vec{v}^1, \dots, \vec{v}^N\right\}$ by bounding $N_p(\beta, \pazocal{M}|_{\sample})$, where $\pazocal{M}|_{\sample}$ is the set of vectors \[\pazocal{M}|_{\sample} = \left\{\left(\profit_M\left(\vec{v}^1\right), \profit_M\left(\vec{v}^2\right), \dots, \profit_M\left(\vec{v}^N\right)\right) \ | \ M \in \pazocal{M}\right\}.\] To finish the proof, we will need a few more theorems and lemmas, which we translate into the language of mechanism design.

\begin{theorem}[\cite{Anthony09:Neural}]\label{thm:pdim_covering}
Let $\pazocal{M}$ be a mechanism class with finite pseudo-dimension $Pdim(\pazocal{M})$ such that for any $M \in \pazocal{M}$ and any valuation vector $\vec{v}$ in the support of $\dist$, $\profit_M(\vec{v}) \in [0,1]$. Then for any set $\sample$, $N_2(\beta, \pazocal{M}|_{\sample}) \leq 2\left(\frac{4e}{\beta^2}\right)^{Pdim(\pazocal{M})}$.
\end{theorem}

\begin{theorem}[\cite{Dudley87:Universal}]\label{thm:dudley}
Let $\pazocal{M}$ be a mechanism class. For any set $\sample$, \[\epsilon_{\pazocal{M}}(N, \delta) \leq 12 \int_0^{\infty} \sqrt{\frac{\log N_2(\beta, \pazocal{M}|_{\sample})}{N}} \, d\beta.\]
\end{theorem}

\begin{lemma}\label{lemma:scale}
For any set of vectors $A \subseteq \R^N$, scalar $c > 0$, and vector $\vec{a}_0 \in \R^N$, we have that $\forall \beta > 0$, $N_p(\beta, \left\{c\vec{a} + \vec{a}_0 : \vec{a} \in A\right\}) \leq N_p(\beta/c, A)$.
\end{lemma}
\begin{proof}
Suppose that $A'$ is a $\beta$-cover of $\left\{c\vec{a} + \vec{a}_0 : \vec{a} \in A\right\}$ in the $L_p$-norm. Then for all $\vec{a} \in A$, there exists $\vec{a}' \in A'$ such that \[\sqrt[p]{\frac{1}{m}\sum_{i = 1}^m (ca_i + a_{0,i} - a_i')^p} \leq \beta.\] Therefore, \begin{align*}\sqrt[p]{\frac{1}{m}\sum_{i = 1}^m (ca_i + a_{0,i} - a_i')^p} &= \sqrt[p]{\frac{1}{m}\sum_{i = 1}^m c^p\left(a_i + \frac{1}{c}(a_{0,i} - a_i')\right)^p}\\
&= c\sqrt[p]{\frac{1}{m}\sum_{i = 1}^m \left(a_i - \frac{1}{c}(a_i' - a_{0,i})\right)^p} \leq \beta. \end{align*} This means that the set $\left\{\frac{1}{c}(\vec{a}' - \vec{a}_0) : \vec{a}' \in A'\right\}$ is a $\frac{\beta}{c}$-cover of $A$.
\end{proof}

We are now ready to bound $\epsilon_{\pazocal{M}}(N, \delta)$ in terms of the pseudo-dimension of $\pazocal{M}$.
Let $\pazocal{M}'|_{\sample} \subseteq [0,1]^N$ be the set of vectors $\pazocal{M}'|_{\sample} = \left\{\frac{1}{U}\vec{w} \ | \ \vec{w} \in \pazocal{M}|_{\sample}\right\}$. The theorem follows from the following chain of inequalities:
\begin{align}
\epsilon_{\pazocal{M}}(N, \delta) &\leq 12 \int_0^{\infty} \sqrt{\frac{\log N_2 \left(\beta, \pazocal{M}|_{\sample}\right)}{N}} \, d\beta \label{ineq:dudley}\\
&\leq \frac{12}{\sqrt{N}} \int_0^{\infty} \sqrt{\log N_2 \left(\frac{\beta}{U}, \pazocal{M}'|_{\sample}\right)} \, d\beta \label{ineq:scale}\\
&\leq \frac{12}{\sqrt{N}} \int_0^{U} \sqrt{\log N_2 \left(\frac{\beta}{U}, \pazocal{M}'|_{\sample}\right)} \, d\beta \label{ineq:int}\\
&\leq \frac{12}{\sqrt{N}} \int_0^{U} \sqrt{\log 2 + Pdim(\pazocal{M})\log\frac{4e}{(\beta/U)^2}} \, d\beta\label{ineq:pdim}\\
&= \frac{12}{\sqrt{N}} \int_0^{U} \sqrt{1 + Pdim(\pazocal{M})\log\frac{4U^2e}{\beta^2}} \, d\beta\\
&\leq \frac{12}{\sqrt{N}}\left(U + \sqrt{Pdim(\pazocal{M})}\int_0^{U} \sqrt{\log\frac{4U^2e}{\beta^2}} \, d\beta\right)\\
&= \frac{12}{\sqrt{N}}\left(U + \sqrt{Pdim(\pazocal{M})}\int_0^{U} \sqrt{\log (4e) + \log\frac{U^2}{\beta^2}} \, d\beta\right)\\
&\leq \frac{12}{\sqrt{N}}\left(U\left(1 + \sqrt{Pdim(\pazocal{M})\log (4e)}\right) + \sqrt{Pdim(\pazocal{M})}\int_0^{U} \sqrt{\log\frac{U^2}{\beta^2}} \, d\beta\right)\\
&= \frac{12}{\sqrt{N}}\left(U\left(1 + \sqrt{Pdim(\pazocal{M})}\left(\sqrt{\log (4e)} +\sqrt{\frac{\pi}{\ln 4}}\right)\right)\right)\\
&\leq \frac{12 U}{\sqrt{N}} \left(1 + 4\sqrt{Pdim(\pazocal{M})}\right)\\
&\leq \frac{12\cdot 5 U}{\sqrt{N}} \sqrt{Pdim(\pazocal{M})}= \frac{60 U}{\sqrt{N}} \sqrt{Pdim(\pazocal{M})},
\end{align} as claimed. Inequality~\eqref{ineq:dudley} follows from Theorem~\ref{thm:dudley}. Inequality~\eqref{ineq:scale} follows from Lemma~\ref{lemma:scale}. Inequality~\eqref{ineq:int} follows from the fact that $\pazocal{M}'|_{\sample} \subseteq [0,1]^N$ which means that  the set $\{\vec{0}\}$ is a $\beta$-cover of $\pazocal{M}'|_{\sample}$ for $\beta \geq 1$, so $\log N_2(\beta, \pazocal{M}|_{\sample}) = 0$. Therefore, we only need to extend the integral to $U$. Inequality~\eqref{ineq:pdim} follows from Theorem~\ref{thm:pdim_covering}. The remaining equalities and inequalities follow from simple algebraic manipulations.
\end{proof}



==> tables.tex <==
\begin{table}
	\scriptsize
	\begin{minipage}{\columnwidth}
		\begin{center}
			\begin{tabularx}{\textwidth}{L{0.55} L{1.7} L{0.1} L{1.25} L{1.4}}
				\toprule
				\textbf{Valuations} & \textbf{Auction class} & & \textbf{Our bounds} & \textbf{Prior bounds}\\\midrule
				Additive or unit-demand  & Length-$\ell$ lottery menu && $U\sqrt{\ell m \log (\ell m)/N}$ & N/A\\\midrule
				Additive, item-independent\footnotemark[1] &  Length-$\ell$ item lottery menu  && $U\sqrt{\ell \log \ell /N}$ & N/A\\\bottomrule
			\end{tabularx}
			\subcaption{Generalization bounds in big-$\tilde O$ notation for lotteries.}
			\begin{tabularx}{\textwidth}{L{0.55} L{1} L{0.8} L{1.25} L{1.4}}
				\toprule
				\textbf{Valuations} & \textbf{Mechanism class} & \textbf{Price class} & \textbf{Our bounds} & \textbf{Prior bounds} \\\midrule
				General & \multirow{2}{*}{\specialcell{Length-$\ell$ menus of\\two-part tariffs\\over $\kappa$ units}} & Anonymous & $U\sqrt{\ell \log (\kappa n\ell)/N}$ &N/A\\\cmidrule{3-5}
				& & Non-anonymous & $U\sqrt{n\ell \log (\kappa n\ell)/N}$ &N/A\\\cmidrule{2-5}
				& \specialcell{Non-linear pricing} & Anonymous & $U\sqrt{m\prod_{i = 1}^m (\kappa_i + 1)/N}$\footnotemark[2]\footnotemark[3] &N/A\\\cmidrule{3-5}
				& & Non-anonymous & $U\sqrt{nm\prod_{i = 1}^m (\kappa_i + 1)/N}$\footnotemark[2]\footnotemark[3] &N/A\\\cmidrule{2-5}
				& \multirow{2}{*}{\specialcell{Additively\\decomposable\\non-linear pricing}} & Anonymous & $U\sqrt{m\sum_{i = 1}^m \kappa_i/N}$\footnotemark[2]\footnotemark[3] &N/A\\\cmidrule{3-5}
				& & Non-anonymous & $U\sqrt{nm\sum_{i = 1}^m \kappa_i/N}$\footnotemark[2]\footnotemark[3] &N/A\\\cmidrule{2-5}
				& Item-pricing & Anonymous & $U\sqrt{m^2/N}$& $U\sqrt{m^2/N}$\footnotemark[4]\\\cmidrule{3-5}
				& & Non-anonymous & $U\sqrt{nm(m + \log n)/N}$ & $U\sqrt{nm^2\log n/N}$\footnotemark[4]\\\midrule
				Unit-demand & Item-pricing & Anonymous & $U\sqrt{m \cdot \min\{m, \log (nm)\}/N}$& $U\sqrt{m^2/N}$\footnotemark[4]\\\cmidrule{3-5}
				& & Non-anonymous & $U\sqrt{nm \log (nm)/N}$ & $U\sqrt{nm^2\log n/N}$\footnotemark[4]\\\midrule
				Additive & Item-pricing & Anonymous & $U\sqrt{m \log m/N}$& $U\sqrt{m \log m/N}$\footnotemark[4], $\left(U/\delta\right)\sqrt{m\log\left(nN\right)/N}$\footnotemark[7]\\\cmidrule{3-5}
				& & Non-anonymous & $U\sqrt{nm \log (nm)/N}$ & $U\sqrt{nm \log (nm)/N}$\footnotemark[4], $\left(U/\delta\right)\sqrt{nm\log \left(N\right)/N}$\footnotemark[7]\\\midrule
				\multirow{2}{*}{\specialcell{Additive,\\item-\\independent\footnotemark[1]}} & Item-pricing & Anonymous & $U\sqrt{1/N}$& $U\sqrt{m \log m/N}$\footnotemark[4], $\left(U/\delta\right)\sqrt{m\log\left(nN\right)/N}$\footnotemark[7]\\\cmidrule{3-5}
				& & Non-anonymous& $U\sqrt{n \log n/N}$ & $U\sqrt{nm \log (nm)/N}$\footnotemark[4], $\left(U/\delta\right)\sqrt{nm\log \left(N\right)/N}$\footnotemark[7]\\\bottomrule
			\end{tabularx}
			\subcaption{Generalization bounds in big-$\tilde O$ notation for pricing mechanisms.}
			\begin{tabularx}{\textwidth}{L{0.55} L{1.8} L{0} L{1.25} L{1.4}}
				\toprule
				\textbf{Valuations} & \textbf{Auction class} && \textbf{Our bounds} & \textbf{Prior bounds}\\\midrule
				General & AMAs and $\lambda$-auctions && $U\sqrt{n^{m+1}m\log n/N}$ & $cU\sqrt{m/N} n^{m+2}\left(n^2 + \sqrt{n^m}\right)$\footnotemark[2]\footnotemark[5]\footnotemark[6]\\\cmidrule{2-5}
				& VVCAs && $U\sqrt{n^2m2^m\log n/N}$ & $cU\sqrt{m/N} n^{m+2}\left(n^2 + \sqrt{n^m}\right)$\footnotemark[2]\footnotemark[5]\footnotemark[6]\\\cmidrule{2-5}
				&MBARPs &&$U \sqrt{m(\log n + m)/N}$&$U \sqrt{m^3 \log n/N}$\footnotemark[5]\\\midrule
				Additive & Second price item auctions with anonymous reserve prices &&$U\sqrt{m \log m/N}$ &$U\sqrt{m \log m/N}$\footnotemark[4]\\\cmidrule{2-5}
				& Second price item auctions with non-anonymous reserve prices &&$U\sqrt{nm \log (nm)/N} $ &$U\sqrt{nm \log (nm)/N}$\footnotemark[4]\\\midrule
				\multirow{2}{*}{\specialcell{Additive,\\item-\\independent\footnotemark[1]}} & Second price item auctions with anonymous reserve prices &&$U\sqrt{1/N}$ &$U\sqrt{m \log m/N}$\footnotemark[4]\\\cmidrule{2-5}
				& Second price item auctions with non-anonymous reserve prices &&$U\sqrt{n \log n/N} $ &$U\sqrt{nm \log (nm)/N}$\footnotemark[4]\\\bottomrule
			\end{tabularx}
			\subcaption{Generalization bounds in big-$\tilde O$ notation for auction classes.}
		\end{center}
	\end{minipage}
	
	\noindent\par
	{\center
		\scriptsize
		\footnotemark[1]~~{Additive cost function};\quad
		\footnotemark[2]~~{Ignoring log factors};\quad
		\footnotemark[6]~~{The value of $c > 1$ depends on the range of the auction parameters};\newline
		\footnotemark[4]~~{\citet{Morgenstern16:Learning}};\quad
		\footnotemark[5]~~{\citet{Balcan16:Sample}};\quad
		\footnotemark[3]~~{$\kappa_i$ is an upper bound on the number of units available of item $i$.}
		\footnotemark[7]~~{\citet{Syrgkanis17:Sample}. The probability these bounds fail to hold is $\delta$. In all other bounds, $\delta$ appears in a log so we suppress it using big-$\tilde O$ notation.}
	}
	\smallskip
	\caption{Our generalization bounds.}\label{tab:results_app}
\end{table}%
